WISK: A Workload-aware Learned Index for Spatial Keyword Queries

Spatial objects often come with textual information, such as Points of Interest (POIs) with their descriptions, which are referred to as geo-textual data. To retrieve such data, spatial keyword queries that take into account both spatial proximity and textual relevance have been extensively studied. Existing indexes designed for spatial keyword queries are mostly built based on the geo-textual data without considering the distribution of queries already received. However, previous studies have shown that utilizing the known query distribution can improve the index structure for future query processing. In this paper, we propose WISK, a learned index for spatial keyword queries, which self-adapts for optimizing querying costs given a query workload. One key challenge is how to utilize both structured spatial attributes and unstructured textual information during learning the index. We first divide the data objects into partitions, aiming to minimize the processing costs of the given query workload. We prove the NP-hardness of the partitioning problem and propose a machine learning model to find the optimal partitions. Then, to achieve more pruning power, we build a hierarchical structure based on the generated partitions in a bottom-up manner with a reinforcement learning-based approach. We conduct extensive experiments on real-world datasets and query workloads with various distributions, and the results show that WISK outperforms all competitors, achieving up to 8x speedup in querying time with comparable storage overhead.

==> sections/acknowledgements.tex <==
This work was partially supported by 
Australian Research Council (ARC) Discovery Project DP230101534, Australian Research Council Future Fellowship FT210100303.
This work was also supported in part by NSFC under Grant 62102341, Basic and Applied Basic Research Fund in Guangdong Province under Grant 2022A1515010166, Shenzhen Science and Technology Program under Grants JCYJ20220530143602006 and ZDSYS20211021111415025, and Guangdong Talent Program under Grant 2021QN02X826. 
The authors would like to thank the anonymous reviewers for providing constructive feedback and valuable suggestions.
